CopyrightMeter: Revisiting Copyright Protection in Text-to-image Models

Text-to-image diffusion models have emerged as powerful tools for generating high-quality images from textual descriptions. However, their increasing popularity has raised significant copyright concerns, as these models can be misused to reproduce copyrighted content without authorization. In response, recent studies have proposed various copyright protection methods, including adversarial perturbation, concept erasure, and watermarking techniques. However, their effectiveness and robustness against advanced attacks remain largely unexplored. Moreover, the lack of unified evaluation frameworks has hindered systematic comparison and fair assessment of different approaches. To bridge this gap, we systematize existing copyright protection methods and attacks, providing a unified taxonomy of their design spaces. We then develop CopyrightMeter, a unified evaluation framework that incorporates 17 state-of-the-art protections and 16 representative attacks. Leveraging CopyrightMeter, we comprehensively evaluate protection methods across multiple dimensions, thereby uncovering how different design choices impact fidelity, efficacy, and resilience under attacks. Our analysis reveals several key findings: (i) most protections (16/17) are not resilient against attacks; (ii) the "best" protection varies depending on the target priority; (iii) more advanced attacks significantly promote the upgrading of protections. These insights provide concrete guidance for developing more robust protection methods, while its unified evaluation protocol establishes a standard benchmark for future copyright protection research in text-to-image generation.

==> related_work.tex <==
  \section{Related Work}

\subsection{Data level}

% Adversarial Perturbations Cannot Reliably Protect Artists From Generative AI

\naen{\textbf{Style mimicry.} Style mimicry uses text-to-image diffusion models to generate images matching a target artistic style. An common method is to finetune a diffusion model by Dreambooth or LoRA using a few images in the targeted style. And models can learn to mimic the style of specific artists after fine-tuning on samples of their art. Some artists concern regarding the potential misuse of style minicry, which could lead to unauthorized replication of their creations.}

\naen{\textbf{Defenses -- Style mimicry protections.} To prevent unauthorized style minicry, many protection methods have been proposed to prevent unauthorized style mimicry by adding small perturbations in their artworks before publishing to disrupt style mimicry methods. }

\naen{\textbf{Attacks -- Circumventing style mimicry protections.} Adversarial purification\cite{yoon2021adversarial} can be used to remove the perturbations introduced by style mimicry protections to circumvent style mimicry protections.}

\subsection{Model level}

% Forget-Me-Not: Learning to Forget in Text-to-Image Diffusion Models
% Circumventing Concept Erasure Methods For Text-to-Image Generative Models

\naen{\textbf{Model Unlearning. } The unlearning problem of deep learning models has become a prevalent academic concern. Significant advances in text-to-image generation models have prompted global discussions on privacy, copyright, and safety. Many models have learned unauthorized personal IDs, content, artistic creations, and potentially harmful materials, later using them to generate uncontrolled content, incuring potential risk of privacy leakage and copyright infringement. }

\naen{\textbf{Defenses -- Concept Forgetting.} Concept forgetting is designed to remove specified sensitive concepts such as objects, or styles from text-to-image models without impairing its ability to generate other content.}

\naen{\textbf{Attacks -- Circumventing Concept Forgetting.} In order to explore whether the model has truly forgotten a concept and to evaluate the effectiveness of the model's forgetting of that concept, many approaches\cite{gal2022image,ruiz2023dreambooth,hu2021lora,tsai2023ring,pham2023circumventing} have been proposed to retrieve ``erased'' concepts from the sanitized models.}

\subsection{Output level}

% Gaussian Shading: Provable Performance-Lossless Image Watermarking for Diffusion Models

\naen{\textbf{Image Watermarking.} Digital watermarking works by embedding copyright or traceable identification information within carrier data, which is an effective approach for copyright protection.}

\naen{\textbf{Defenses -- Image Watermarking for Diffusion Models.} Prior to the advent of diffusion models, traditional image watermarking methods directly modify the image, thus degrading image quality, which is called post-processing-based watermarks. With the emergence of diffusion models, recent research endeavors to integrate the watermark embedding process with the image generation process to mitigate this issue.}

\naen{\textbf{Attacks -- Removing Image Watermark.} To assess the robustness of the watermarking techniques, adding post-processing perturbations of watermarked images could be employed to degrade or remove invisible embedded watermarks. }

\subsection{Overview}

\naen{Some recent studies \cite{ren2024copyright,pham2023circumventing,honig2024adversarial} have surveyed copyright defenses/attacks; yet, none of them provides benchmark implementation or empirical evaluation to explore their strengths/limitations from both data, model, and output-level. \cite{ren2024copyright} introduces methodology in two aspects --  data-level copyright protection held by data owners and model-level copyright protection by model builders; however, it does not experiment with these methods or measure the quality of the generated images. \cite{honig2024adversarial} focuses on data-level artistic style imitation, demonstrating that all existing copyright protections can be easily bypassed through a user study, leaving artists vulnerable to style mimicry. However, aside from user studies, the paper did not employ image quality-related evaluation metrics. \cite{pham2023circumventing} focus on model-level concept erasure methods, and proposed concept inversion methods for each specific model forgetting approach to relearn the forgotten concepts. However, the paper did not consider contrasting the proposed method with other relearning methods.}
